Reconfigurable Quantum Instruction Set Computers for High Performance Attainable on Hardware

The performance of current quantum hardware is severely limited. While expanding the quantum ISA with high-fidelity, expressive basis gates is a key path forward, it imposes significant gate calibration overhead and complicates compiler optimization. As a result, even though more powerful ISAs have been designed, their use remains largely conceptual rather than practical. To move beyond these hurdles, we introduce the concept of "reconfigurable quantum instruction set computers" (ReQISC), which incorporates: (1) a unified microarchitecture capable of directly implementing arbitrary 2Q gates equivalently, i.e., SU(4) modulo 1Q rotations, with theoretically optimal gate durations given any 2Q coupling Hamiltonians; (2) a compilation framework tailored to ReQISC primitives for end-to-end synthesis and optimization, comprising a program-aware pass that refines high-level representations, a program-agnostic pass for aggressive circuit-level optimization, and an SU(4)-aware routing pass that minimizes hardware mapping overhead. We detail the hardware implementation to demonstrate the feasibility, in terms of both pulse control and calibration of this superior gate scheme on realistic hardware. By leveraging the expressivity of SU(4) and the time minimality realized by the underlying microarchitecture, the SU(4)-based ISA achieves remarkable performance, with a 4.97-fold reduction in average pulse duration to implement arbitrary 2Q gates, compared to the usual CNOT/CZ scheme on mainstream flux-tunable transmons. Supported by the end-to-end compiler, ReQISC outperforms the conventional CNOT-ISA, SOTA compiler, and pulse implementation counterparts, in significantly reducing 2Q gate counts, circuit depth, pulse duration, qubit mapping overhead, and program fidelity losses. For the first time, ReQISC makes the theoretical benefits of continuous ISAs practically feasible.

==> algorithms/mirroring_sabre.tex <==
% \documentclass{article}
% \usepackage[ruled, vlined, linesnumbered]{algorithm2e}
% \usepackage{amsmath}
% \usepackage{mhchem}
% \usepackage{xcolor}
% \usepackage{amssymb}

% \begin{document}
       \begin{algorithm}[tbp]
       \SetAlgoLined
       \caption{Mirroring-SABRE's Heuristic $\mathrm{SWAP}$ Search \textit{(partial)}}
       \label{algo:mirroring_sabre}
       \SetKwInOut{Input}{Input}
       \SetKwInOut{Output}{Output}
       \SetKwBlock{Assumption}{Assumption}{}
   
       % \Input{Pauli strings with corresponding coefficients (\textit{pls}, \textit{coes})}
       \Input{Front layer $F$, Extended set $E$, Last mapped layer $ L $, Mapping $\pi$, Distance matrix $D$, Weight coefficient $W$,  Circuit DAG, Qubit coupling graph $G(V,E)$}
       \Output{Inserted $ \mathrm{SWAP} $,  Updated mapping $ \pi $}
       % \tcp{Following pseudocode only involves transformation on pls while omitting coes WLOG}
       % $ F \gets$ Font layer\;
       % $ L \gets$ Last mapped layer\;
       % $H_0 := \frac{1}{\left|{F}\right|} \sum_{gate \in F} D[\pi(gate.q_1)] \pi(gate.q2)] + \frac{W}{\left|{E}\right|} \sum_{gate \in E} D[\pi(gate.q_1)][\pi(gate.q2)].$\;
       \BlankLine
       $H_0 \coloneqq \frac{1}{\left|{F}\right|} \sum_{g \in F} D[\pi(g.q_1), \pi(g.q_2)] + \frac{W}{\left|{E}\right|} \sum_{g \in E} D[\pi(g.{q_1}),\pi(g.{q_2})]$\label{line:H0}\;
       \textit{SWAP\_candidate\_list} $\gets$ \textsc{ObtainCandidateSWAPs}$(F,G)$\;
       $\textit{cost}_0 \gets H_0(F, \text{DAG}, \pi, D) $\;
       \For{$ \mathrm{SWAP} $ \textbf{in} \textit{SWAP\_candidate\_list}}{
           $ \pi_{\text{temp}} \gets \pi.\textsc{update}(\mathrm{SWAP}) $\;
           $ \textit{cost}[\mathrm{SWAP}] \gets H(F, \text{DAG}, \pi_{\text{temp}}, D, \mathrm{SWAP}) $\;
       }
       
       $ \mathrm{SWAP}\gets$ Find the minimal-cost $ \mathrm{SWAP} $ from \textit{SWAP\_candidate\_list} which can be absorbed by $ L $ and leads to less cost than $\textit{cost}_0$\;
       %  \gets \textsc{FindMinimalcostSWAP}(\textit{cost}, L) $\;
       \If{$ \mathrm{SWAP} = \emptyset $}{
           $ \mathrm{SWAP} \gets $ Find the $ \mathrm{SWAP} $ with minimal cost\;
       }
       $ \pi \gets \pi.\textsc{update}(\mathrm{SWAP}) $\;
       \end{algorithm}
    %    \Description[Mirroring-SABRE's Heuristic $\mathrm{SWAP}$ Search.]{Mirroring-SABRE's Heuristic $\mathrm{SWAP}$ Search.}

   % \end{document}
   
